A Search-Based Framework for Automatic Generation of Testing Environments for Cyber-Physical Systems

Many modern cyber physical systems incorporate computer vision technologies, complex sensors and advanced control software, allowing them to interact with the environment autonomously. Testing such systems poses numerous challenges: not only should the system inputs be varied, but also the surrounding environment should be accounted for. A number of tools have been developed to test the system model for the possible inputs falsifying its requirements. However, they are not directly applicable to autonomous cyber physical systems, as the inputs to their models are generated while operating in a virtual environment. In this paper, we aim to design a search based framework, named AmbieGen, for generating diverse fault revealing test scenarios for autonomous cyber physical systems. The scenarios represent an environment in which an autonomous agent operates. The framework should be applicable to generating different types of environments. To generate the test scenarios, we leverage the NSGA II algorithm with two objectives. The first objective evaluates the deviation of the observed system behaviour from its expected behaviour. The second objective is the test case diversity, calculated as a Jaccard distance with a reference test case. We evaluate AmbieGen on three scenario generation case studies, namely a smart-thermostat, a robot obstacle avoidance system, and a vehicle lane keeping assist system. We compared three configurations of AmbieGen: based on a single objective genetic algorithm, multi objective, and random search. Both single and multi objective configurations outperform the random search. Multi objective configuration can find the individuals of the same quality as the single objective, producing more unique test scenarios in the same time budget.

==> Makefile <==
PAPER="main"
TARGET=ist-2021

CC=latex
CC=pdflatex
READER=acroread
READER=open # no easy way so far to hack the mac ...


SHELL=bash

$(PAPER).pdf: clean compile *.tex *.bib # figures/*.eps
	cp  $(PAPER)".pdf" $(TARGET).pdf 
#	cp  $(PAPER)".pdf"  ~/GoogleDrive/GiulioPrivate/ReadAndMark/$(TARGET).pdf
	$(READER) main.pdf


compile: *.tex *.bib # figures/*.eps
	$(CC) $(PAPER)
	bibtex $(PAPER)
	$(CC) $(PAPER) # I love space in file names!
	$(CC) $(PAPER)
	#now loop over Latex file, until stable (use zot to deal with annoying OS):
	echo Zot > $(PAPER).log
	while grep Zot $(PAPER).log >/dev/null 2>&1 ; do $(CC) $(PAPER).tex ; done
	if [ $(CC) = "latex" ]	; then\
	   	dvips -t letter $(PAPER) -o $(PAPER).ps ;\
		ps2pdf13 $(PAPER).ps $(PAPER).pdf ;\
		fi

clean:
	rm -f $(PAPER).dvi
	rm -f $(PAPER).ps
	rm -f $(PAPER).pdf
	rm -f $(PAPER).bbl
	rm -f $(PAPER).blg
	rm -f $(PAPER).log
	rm -f $(PAPER).out
	rm -f $(PAPER).aux
	find . -name  "*~" -exec rm {} \;
	find . -name  "*.log" -exec rm {} \;
	find . -name  "*.bak" -exec rm {} \;
	find . -name  "*.aux" -exec rm {} \;
	find . -name  "*.dvi" -exec rm {} \;
	find . -name  "*.blg" -exec rm {} \;
	find . -name  "*.bbl" -exec rm {} \;
	find .  -maxdepth 0 -name  "*.ps" -exec rm {} \;
	find .  -maxdepth 0 -name  "*.pdf"  -exec rm {} \;


#check references:
refcheck:clean
	make compile
	make compile | grep "Reference\|Rerun" | sed 's/LaTeX\ Warning:\ Reference\ //' | tr '`' "'" > latex_refs.log
	make compile | grep Citation >> latex_refs.log ; true
	make compile | grep Label | grep multiply >> latex_refs.log ; true
	if [ -f  latex_refs.log ]	; then\
		echo "Check latex_refs.log:" ;\
		cat latex_refs.log ;\
		else \
		echo "Check Reference Done! No error found!" ;\
	fi
## now commit cnages
git: 
	make clean
	make refcheck
	git commit -m "updated" *.tex *.bib


==> abstract.tex <==
\textbf{Background.} Many modern cyber-physical systems incorporate computer vision technologies, complex sensors and advanced control software, allowing them to interact with the environment autonomously. Examples include drone swarms, self-driving vehicles, autonomous robots, etc. Testing such systems poses numerous challenges: not only should the system inputs be varied, but also the surrounding environment.
\textbf{Aims.} In this research paper, we aim to design a search-based algorithm for generating diverse fault-revealing test cases for autonomous cyber-physical systems. The test cases should account for varying environmental conditions and surroundings, and the algorithm should be applicable to different test case generation goals.
Method. To generate the test cases we are using an NSGA-II algorithm with two objectives. The first objective evaluates the deviation of the observed system behaviour from its expected behaviour for a particular test case. The observed system behaviour is computed using a surrogate system model, while the expected behaviour is specified in the requirements. The second objective is the test case diversity, calculated as a Jaccard distance with a reference test case.
\textbf{Results.} We evaluate our approach on three problems, namely a smart-thermostat, a vehicle lane-keeping assist system, and a robot obstacle avoidance system. For all the problems, our approach outperforms baseline approaches in fault revealing and several other metrics such as the diversity of the revealed faults and the proportion of the valid test scenarios.
\textbf{Conclusions.} Adding a second objective, accounting for diversity, allows producing test suites with diverse fault revealing cases. For the problems, where one solution is enough we suggest using the single-objective version of our algorithm as it converges faster to a higher fitness value.
%The failures of the real system can be detected using the surrogate model. The number of fault-revealing test cases can be increased by fine-graining the surrogate model on the data collected from simulations with the original system model.

==> algorithms/algorithm1.tex <==


\begin{algorithm}[H]
\caption{Test case generation algorithm}\label{alg:euclid}
\begin{flushleft}
\textbf{Input:}
\setlength{\parindent}{8ex}
- population size $P_s$\\
- crossover rate $C_r$\\
- mutation rate $M_r$\\
- number of offsprings $N$ \\
- termination criteria $T$\\
- fitness functions $F_1$, $F_2$\\
- constraints C
\end{flushleft}
\textbf{Output:} a set of critical scenarios $CS = (TC_1, TC_2, TC_i)$, represented by the Pareto optimal solutions found by the algorithm

\begin{algorithmic}[1]
\Procedure {NSGA2 scenario generation}{$P,C_r, M_r, N$}\\
\quad  {\# Generate an initial population set P randomly\\ \qquad using  a Markov chain}
\State $population \; \mu \gets PopulationSampling(P_s)$
%\Comment{We have the answer if r is 0}
\State $Evaluate(\mu, F_1, F_2)$\\
\qquad \#{while termination criteria is not reached}
\While{not ($T$) }\\
\quad \qquad {\# select offsprings for crossover and mutation}
\State {$offsprings \; Q \gets BinaryTournament(N, \mu)$}
\State {$children \; \lambda \gets OnePointCrossover(Q, C_r)$}
\State {$children \; \lambda \gets Mutation(\lambda, M_r)$}\\
\quad \qquad {\# add offsprings to the population}
\State {$population \; \mu \gets \mu + \lambda$}
%\State \textbf{$Foreach \; q \in Q$}
\State $Evaluate(\mu, F_1, F_2)$\\
\quad \qquad {\# update the population by selecting top $P_s$ } \\ \quad \qquad {individuals from the old population and offsprings}
\State $population \; \mu \gets UpdatePopulation(P_s)$

\EndWhile\label{euclidendwhile}

\State \textbf{return} $CS$
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> ev1.tex <==

\subsubsection{Experimental set-up}
 

\begin{figure}[ht]
\includegraphics[scale=0.27]{images/thermostat_results.PNG}
\centering
\caption{Fitness function value over evaluations for the thermostat case study}
\centering
\label{fig:therm_res}
%\vspace{-5mm}
\end{figure}
We are using a high mutation rate, as from our experience, it allowed to converge to better solutions faster. In our implementation a $\mu$+$\lambda$ insertion approach is used, where only the best individuals from previous generation and offsprings are inserted to the next generation. Therefore, with mutation  only broaden the search space as the individuals with lower fitness after mutation are discarded. In the generational GA the number of offsprings inserted in the population is equal to the population size.  

The average time to run 50000 evaluations was 136.691 sec for GA and 123.665 sec for NSGA-II. 
\subsubsection{Results}
In the Fig. \ref{fig:therm_res} we present the best fitness value found over generations by Random search(green boxplots), GA(red boxplots) and NSGA-II (blue boxplots) averaged over 30 runs. We considered the fitness function described in (\ref{f1}).
We statistically compare the fitness function values found after 50000 evaluations with a two-tailed non-parametric Mann-Whitney U test. The obtained p values and effect sizes are shown in the table \ref{tab:therm_p}. 
\input{tables/therm_p}
%\input{tables/therm_d}

We can see that GA and NSGA-II find significantly better solutions, than the random search.  GA and NSGA-II show no statistical difference in the produced solutions. %However,  GA on average converges faster to a certain fitness value, than NSGA2.

In the Fig. \ref{fig:div_therm} we compare how diverse are the produced solutions by GA and NSGA-II.
For GA, we select the fittest individual and compute $F_{2therm}$ between it and the other four fittest individuals.
For NSGA-II, we select one solution from the Pareto front and compute  $F_{2therm}$ between it and other Pareto optimal solutions. The size of the Pareto front was 7 individuals on average. All the solutions in the Pareto front have a $F_{1therm}$ value higher than a certain fault-revealing threshold, established by the developer.

The two-tailed non-parametric Mann-Whitney U test confirms with a p value smaller than 0.01 that NSGA-II produces more diverse solutions, with a "large" effect size of 0.852.
\begin{figure}[h!]
\includegraphics[scale=0.28]{images/novelty_thermostat.PNG}
\centering
\caption{Novelty of the test cases in the last generation}
\centering
\label{fig:div_therm}
%\vspace{-5mm}
\end{figure}

\subsubsection{Test case examples}
Finally, we discuss an example of the produced scenarios.
In the Fig.\ref{fig:tc-first} you can see a scenario with a low fitness value of 0.76 degrees, indicating that the temperature deviates from the schedule 0.76 degrees on average. On the contrary, in  Fig.\ref{fig:tc-second} the scenario produced by the NSGA-II search has a higher fitness of 2.4 degrees. Clearly, this scenario is more likely to be unacceptable to the user, comparing to the first one.

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[scale=0.13]{images/20.png}  
  \caption{Randomly produced scenario}
  \label{fig:tc-first}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include third image
  \includegraphics[scale=0.13]{images/10.png}  
  \caption{Search produced scenario}
  \label{fig:tc-second}
\end{subfigure}

\caption{Examples of scenarios for the smart thermostat}
\label{fig:fig_tc_therm}
\end{figure}


==> ev2.tex <==
\subsubsection{Experimental set-up}
We used the following GA and NSGA configurations:
population size: 500, 
number of generations: 200,
mutation rate: 0.4,
crossover rate: 1,
algorithm type: generational,
number of evaluations: 100 000.
\begin{figure}[ht]
\includegraphics[scale=0.27]{images/vehicle_results2.PNG}
\centering
\caption{Fitness function value over evaluations for the vehicle case study}
\centering
\label{fig:veh_res}
%\vspace{-5mm}
\end{figure}

We are using a higher population size, rather than the bigger number of generations, as from our experience, with bigger population the results were more consistent across different runs. 
 
The average time to run 100000 evaluations was 1522.405 sec for GA and 1380.66 sec for NSGA-II. 

\subsubsection{Results}
In the Fig. \ref{fig:veh_res} we present the best fitness value found over generations by Random search (green boxplots), GA (red boxplots) and NSGA-II (blue boxplots) averaged over 30 runs. We considered the fitness function described in (\ref{f1}).
We statistically compare the fitness function values found after 100 000 evaluations with a two-tailed non-parametric Mann-Whitney U test. The obtained p values and effect sizes are shown in the table \ref{tab:veh_p}. The corresponding Cliff's delta values are shown in table \ref{tab:veh_d}.

\input{tables/vehicle_p}

%\input{tables/vehicle_d}

We can see that GA and NSGA-II find significantly better solutions, than the random search.  However, we have a high probability of error rejecting the null hypothesis that GA and NSGA-II come from different distributions. Therefore we cannot say with 95 \% confidence that GA converges to better solutions.

\begin{figure}[h]
\includegraphics[scale=0.27]{images/novelty_car.PNG}
\centering
\caption{Novelty of the test cases in the last generation}
\centering
\label{fig:div_car}
%\vspace{-5mm}
\end{figure}

In the Fig. \ref{fig:div_car} we compare how diverse are the produced solutions by GA and NSGA-II.
For GA, we select the fittest individual and compute $F_{2veh}$ between it and the other four fittest individuals.
For NSGA-II, we select one solution from the Pareto front and compute  $F_{2veh}$ between it and other Pareto optimal solutions. The size of the Pareto front was 7 individuals on average. All the solutions in the Pareto front have a $F_{1veh}$ value higher than a certain fault-revealing threshold, established by the developer.


The two-tailed non-parametric Mann-Whitney U test confirms with a p=0.015 ($p \leq 0.05$) that NSGA-II produces more diverse solutions, with a "medium" effect size of 0.363.

\subsubsection{Comparison with baselines}
In this subsection we report results of evaluating  our NSGA-II based approach and the Frenetic tool (frenetic). In addition we evaluate the random search (RS), guided by our fitness function (\ref{f1}), and  the random generator (random).

For our NSGA-II we used a simplified configuration:
population  size:  90,  number  of  generations: 200, mutation rate: 0.4, crossover rate: 1, number of offsprings: 25, number of evaluations: 5090.
We used the simplified version to produce more test cases given a limited time budget for evaluation (2 hours). We gave the same time budget (5090 evaluations) for the random search to produce the solutions.

Approaches are evaluated using the SBST2021 code pipeline, that integrates the test generators with the  BeamNG simulator by validating, executing and evaluating the generated test cases.  We executed the SBST21 2 hour experiment, where the fault is revealed when 0.85 percent of the car area goes out of the lane. Also, the driving agent travels up to 70 Km/h.

The test cases are compared in terms of the number of faults Fig. \ref{fig:obe_car}, the diversity of the faults Fig. \ref{fig:spars_car} and the proportion of the valid test cases Fig.\ref{fig:valid_car}.
The corresponding statistical test and effect size measures (Cliff's delta) are shown in the tables \ref{tab:obe}, \ref{tab:spars} and \ref{tab:ratio}.

\begin{figure}[h!]
\includegraphics[scale=0.27]{images/obe.PNG}
\centering
\caption{The number of revealed faults}
\centering
\label{fig:obe_car}
%\vspace{-5mm}
\end{figure}


\input{tables/obe}
In terms of the number of the revealed faults both, our approach and Frenetic, statistically outperform the random search and the random generator. Out of 30 runs, on average, Swat and Frenetic produce almost equal amount of faults, i.e. 14.

\begin{figure}[h!]
\includegraphics[scale=0.27]{images/sparsity.PNG}
\centering
\caption{The diversity of the revealed faults}
\centering
\label{fig:spars_car}
%\vspace{-5mm}
\end{figure}

\input{tables/sparsity}

Concerning the diversity of the revealed faults, all the approaches show similar performance and dont't show a statistically significant difference.
\begin{figure}[h!]
\includegraphics[scale=0.27]{images/ratio.PNG}
\centering
\caption{The proportion of the valid test cases}
\centering
\label{fig:valid_car}
%\vspace{-5mm}
\end{figure}


\input{tables/ratio}
Another important factor was  the proportion of valid test cases out of all the cases produced. From the table \ref{tab:ratio} we see that the Swat and random generator produce statistically bigger proportion of the valid test cases, that Frenetic and random search.
In table \ref{tab:tc_number} we also indicate the average number of the total produced test cases as well as the number of invalid and valid test cases.  SBST21 code pipeline evaluates the test cases procedurally, i.e. as soon as the valid test case is produced it is executed. The new test case can only be produced, when the execution of the previous one stops.  The scenario execution time depends on the generated road length i.e. the longer the road, the more time the car will spend in the simulation. Therefore, we do not evaluate the approaches by the total number of the produced scenarios, as it depends not only on the efficiency of the algorithm, but also on the duration of the generated scenarios. The random search generates the lowest number of solutions as it only provides one solution after 5090 evaluations. The swat, on the contrary, provides around 7 solutions on average, corresponding to the search Pareto front after 5090 evaluations. 

\input{tables/total_tc}
\subsubsection{Test case examples}
In the Fig. \ref{fig:fig_roads} we show examples of the generated test cases, that forced the car to go out of the lane.
\begin{figure}[h!]
\begin{subfigure}{.2\textwidth}
  \centering
  % include third image
  \includegraphics[scale=0.21]{images/car_tc_ed1.png}  
  \caption{Car going out of bounds}
  \label{fig:sub-third}
\end{subfigure}
\begin{subfigure}{.2\textwidth}
  \centering
  % include fourth image
  \includegraphics[scale=0.21]{images/car_tc_ed2.png}  
  \caption{Car going out of bonds}
  \label{fig:sub-fourth}
\end{subfigure}
\caption{Examples of fault revealing test cases}
\label{fig:fig_roads}
\end{figure}



==> ev3.tex <==

\subsubsection{Experimental set-up}
We used the following GA and NSGA configurations:
population size: 100, 
number of generations: 400,
mutation rate: 0.4,
crossover rate: 1,
algorithm type: steady state with 10 offsprings,
number of evaluations: 4 000.


\begin{figure}[h!]
\includegraphics[scale=0.26]{images/robot_results3.PNG}
\centering
\caption{Fitness function value over evaluations for the robot case study}
\centering
\label{fig:rob_res}
%\vspace{-5mm}
\end{figure}

For this problem we used a smaller number of offsprings to run more generations for the same time budget. The A* algorithm implementation was computationally expensive to execute.


The average time to run 4000 evaluations was 2168.679 sec for GA and 2001.795 sec for NSGA-II. 
\subsubsection{Results}
In the Fig. \ref{fig:rob_res} we present the best fitness value found over generations by Random search (green boxplots), GA (red boxplots) and NSGA-II (blue boxplots) averaged over 30 runs. We considered the fitness function described in (\ref{f1}).
We statistically compare the fitness function values found after 4000 evaluations with a two-tailed non-parametric Mann-Whitney U test. The obtained p values and effect sizes are shown in the table \ref{tab:rob_p}. 
\input{tables/robot_p}

%\input{tables/robot_d}


In the Fig. \ref{fig:div_rob} we compare how diverse are the produced solutions by GA and NSGA-II.
For GA, we select the fittest individual and compute $F_{2rob}$ between it and the other four fittest individuals.
For NSGA-II, we select one solution from the Pareto front and compute  $F_{2rob}$ between it and other Pareto optimal solutions. The size of the Pareto front was 7 individuals on average. All the solutions in the Pareto front have a $F_{1rob}$ value higher than a certain fault-revealing threshold, established by the developer.

The two-tailed non-parametric Mann-Whitney U test confirms with a p value smaller than 0.01 that NSGA-II produces more diverse solutions, with a "large" effect size of 1.

\begin{figure}[h!]
\includegraphics[scale=0.27]{images/novelty_robot.PNG}
\centering
\caption{Novelty of the test cases in the last generation}
\centering
\label{fig:div_rob}
%\vspace{-5mm}
\end{figure}


\subsubsection{Test case examples}
In the Fig.\ref{fig:fig_maps} we show examples of the generated scenarios i.e. rooms with obstacles by random sampling Fig. \ref{fig:sub-room1} and the search algorithm Fig. \ref{fig:sub-room2}.
In Fig. \ref{fig:sub-room1} the length of the robot path towards the goal is 78.76 meters, while in the Fig. \ref{fig:sub-room1} - 2020.36 meters. Evidently, the second scenario poses a more challenging navigation environment for the robot, than the first scenario.
\begin{figure}[h!]
\begin{subfigure}{.23\textwidth}
  \centering
  % include third image
  \includegraphics[scale=0.17]{images/tc_25.jpg}  
  \caption{A randomly produced scenario}
  \label{fig:sub-room1}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  % include fourth image
  \includegraphics[scale=0.17]{images/tc_3.jpg}  
  \caption{Search produced scenario}
  \label{fig:sub-room2}
\end{subfigure}
\caption{Examples obtained robot navigation maps}
\label{fig:fig_maps}
\end{figure}


==> macro.tex <==
\usepackage{amssymb}
\usepackage{ifthen}
\usepackage{xspace}

\makeatletter



\def\question{\emph{If this particular file changes, what other files should change?}}



\newcommand{\COMMENT}[1]{}
\newcommand{\ndef}{\stackrel{\rm def}{=}}
\newcommand{\minitab}[2][l]{\begin{tabular}{#1}#2\end{tabular}}



\newcommand{\Foutse}[1]{\textcolor{blue}{{\it [Foutse: #1]}}}
\newcommand{\giulio}[1]{\textcolor{blue}{{\it [Giulio says: #1]}}}
\newcommand{\foutse}[1]{\textcolor{red}{{\it [Foputse says: #1]}}}
\newcommand{\cyrin[1]}{\textcolor{magenta}{{\it [Cyrin says: #1]}}}

\newcommand{\Dima}[1]{\textcolor{blue}{{\it  #1}}}


\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}


==> results.tex <==
In this section we provide evaluation results for the considered problems as well the answers to the three research questions.

For all the problems, We implemented the single-objective genetic algorithm (GA) and NSGA-II multi-objective algorithm in python, using the Pymoo framework \cite{pymoo}.

 \subsection{Wireless thermostat problem {\label{sec:case1}}}
\input{ev1}
 \subsection{Lane keeping assist system problem {\label{sec:case2}}}
\input{ev2}
 \subsection{ Autonomous navigating robot  problem{\label{sec:case3}}}
\input{ev3}

==> tables/robot_d.tex <==
\begin{table}[h!]
\begin{center}
\caption{Results of Cliff delta calculation for the robot problem
}
\label{tab:rob_d}
\scalebox{1}{
\begin{tabular}{|c|c|c|c|} 
\hline 
       & $GA$ & $NSGA2$ & $Random$ \\
\hline
$GA$  &   $0 , \; negligible$    &         &           \\
\hline
$NSGA2$ &  $0.772, \; large$  &  $0 , \; negligible$ &   \\
\hline
$Random$ &  $1, \; large$  & $0.978, \; large$ & $0 , \; negligible$  \\
\hline
\end{tabular}}
\end{center}
\end{table}

==> tables/therm_d.tex <==
\begin{table}[ht]
\begin{center}
\caption{Results of Cliff delta calculation}
\label{tab:therm_d}
\scalebox{1}{
\begin{tabular}{|c|c|c|c|} 
\hline 
       & $GA$ & $NSGA2$ & $Random$ \\
\hline
$GA$  &   $0 , \; negligible$    &         &           \\
\hline
$NSGA2$ &  $0.133, \; negligible$  &  $0 , \; negligible$ &   \\
\hline
$Random$ &  $1, \; large$  & $1, \; large$ & $0 , \; negligible$  \\
\hline
\end{tabular}}
\end{center}
\end{table}

==> tables/vehicle_d.tex <==
\begin{table}[h!]
\begin{center}
\caption{Results of Cliff delta calculation for vehicle case study}
\label{tab:veh_d}
\scalebox{1}{
\begin{tabular}{|c|c|c|c|} 
\hline 
       & $GA$ & $NSGA2$ & $Random$ \\
\hline
$GA$  &   $0 , \; negligible$    &         &           \\
\hline
$NSGA2$ &  $0.215, \; small$  &  $0 , \; negligible$ &   \\
\hline
$Random$ &  $0.877, \; large$  & $0.886, \; large$ & $0 , \; negligible$  \\
\hline
\end{tabular}}
\end{center}
\end{table}
